Knowledge Reutilization in Meta-Reinforcement Learning

Meta-reinforcement learning enables fast adaptation by extracting shared structure from related tasks, but existing end-to-end methods often couple task inference with embodiment-specific control. This coupling can obscure non-parametric task semantics, reduce sample efficiency, and limit cross-agent reuse. We propose a meta-knowledge reutilization framework that learns task-level knowledge on a dynamics-simplified agent and transfers it to heterogeneous agents. The framework uses a Bayesian non-parametric prior to organize latent task modes and a high-level policy to generate task-level magnitude guidance. To bridge reusable task knowledge with different embodiments, we introduce a semantic-magnitude interface and a lightweight temporal adaptor, which convert frozen meta-knowledge into temporally aligned subgoals for embodiment-specific low-level controllers. Experiments on multiple locomotion agents show that our framework reduces final-step tracking error by 94.75% -- 99.79% compared with recent state-of-the-art baselines and achieves comparable deployment performance with about 23.8% of their interaction data.

==> img_tex/all_agents__ours_task_inference_results.tex <==
% -- multi-agent DPMM inference trajectories with hardcoded targets --
\newcommand{\PlotDPMMAgentInference}[3]{
\begin{figure}[t!]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tikzpicture}[font=\sffamily]

        % ================= Position tracking =================
        \begin{axis}[
            name=posplot,
            width=10cm,
            height=4.6cm,
            xmin=0, xmax=100,
            ymin=-20, ymax=15,
            ylabel={Position (m)},
            xticklabels=\empty,
        ]

        \addplot[blue!75, line width=0.9pt]
        table[col sep=comma, x expr=\coordindex, y=x_before]
        {data/multi_task_inference_result_dpmm(ours)/#1/smooth/subgoals_ep0_smooth.csv};
        \addplot[blue!75, dashed, line width=0.8pt, opacity=0.55, forget plot]
        coordinates {(0,-9.02) (100,-9.02)};

        \addplot[red!75, line width=0.9pt]
        table[col sep=comma, x expr=\coordindex, y=x_before]
        {data/multi_task_inference_result_dpmm(ours)/#1/smooth/subgoals_ep1_smooth.csv};
        \addplot[red!75, dashed, line width=0.8pt, opacity=0.55, forget plot]
        coordinates {(0,-5.10) (100,-5.10)};

        \addplot[green!60!black, line width=0.9pt]
        table[col sep=comma, x expr=\coordindex, y=x_before]
        {data/multi_task_inference_result_dpmm(ours)/#1/smooth/subgoals_ep2_smooth.csv};
        \addplot[green!60!black, dashed, line width=0.8pt, opacity=0.55, forget plot]
        coordinates {(0,-3.14) (100,-3.14)};

        \addplot[orange!85!black, line width=0.9pt]
        table[col sep=comma, x expr=\coordindex, y=x_before]
        {data/multi_task_inference_result_dpmm(ours)/#1/smooth/subgoals_ep3_smooth.csv};
        \addplot[orange!85!black, dashed, line width=0.8pt, opacity=0.55, forget plot]
        coordinates {(0,3.14) (100,3.14)};

        \addplot[purple!75, line width=0.9pt]
        table[col sep=comma, x expr=\coordindex, y=x_before]
        {data/multi_task_inference_result_dpmm(ours)/#1/smooth/subgoals_ep4_smooth.csv};
        \addplot[purple!75, dashed, line width=0.8pt, opacity=0.55, forget plot]
        coordinates {(0,5.10) (100,5.10)};

        \addplot[cyan!70!black, line width=0.9pt]
        table[col sep=comma, x expr=\coordindex, y=x_before]
        {data/multi_task_inference_result_dpmm(ours)/#1/smooth/subgoals_ep5_smooth.csv};
        \addplot[cyan!70!black, dashed, line width=0.8pt, opacity=0.55, forget plot]
        coordinates {(0,9.02) (100,9.02)};

        \end{axis}

        % ================= Velocity tracking =================
        \begin{axis}[
            at={(posplot.below south west)},
            anchor=above north west,
            yshift=-0.35cm,
            width=10cm,
            height=4.6cm,
            xmin=0, xmax=100,
            ymin=-3.2, ymax=3.2,
            xlabel={Time Step},
            ylabel={Velocity (m/s)},
        ]

        \addplot[blue!75, line width=0.9pt]
        table[col sep=comma, x expr=\coordindex, y=vx_before]
        {data/multi_task_inference_result_dpmm(ours)/#1/smooth/subgoals_ep6_smooth.csv};
        \addplot[blue!75, dashed, line width=0.8pt, opacity=0.55, forget plot]
        coordinates {(0,-2.35) (100,-2.35)};

        \addplot[red!75, line width=0.9pt]
        table[col sep=comma, x expr=\coordindex, y=vx_before]
        {data/multi_task_inference_result_dpmm(ours)/#1/smooth/subgoals_ep7_smooth.csv};
        \addplot[red!75, dashed, line width=0.8pt, opacity=0.55, forget plot]
        coordinates {(0,-1.75) (100,-1.75)};

        \addplot[green!60!black, line width=0.9pt]
        table[col sep=comma, x expr=\coordindex, y=vx_before]
        {data/multi_task_inference_result_dpmm(ours)/#1/smooth/subgoals_ep8_smooth.csv};
        \addplot[green!60!black, dashed, line width=0.8pt, opacity=0.55, forget plot]
        coordinates {(0,-1.45) (100,-1.45)};

        \addplot[orange!85!black, line width=0.9pt]
        table[col sep=comma, x expr=\coordindex, y=vx_before]
        {data/multi_task_inference_result_dpmm(ours)/#1/smooth/subgoals_ep9_smooth.csv};
        \addplot[orange!85!black, dashed, line width=0.8pt, opacity=0.55, forget plot]
        coordinates {(0,1.45) (100,1.45)};

        \addplot[purple!75, line width=0.9pt]
        table[col sep=comma, x expr=\coordindex, y=vx_before]
        {data/multi_task_inference_result_dpmm(ours)/#1/smooth/subgoals_ep10_smooth.csv};
        \addplot[purple!75, dashed, line width=0.8pt, opacity=0.55, forget plot]
        coordinates {(0,1.75) (100,1.75)};

        \addplot[cyan!70!black, line width=0.9pt]
        table[col sep=comma, x expr=\coordindex, y=vx_before]
        {data/multi_task_inference_result_dpmm(ours)/#1/smooth/subgoals_ep11_smooth.csv};
        \addplot[cyan!70!black, dashed, line width=0.8pt, opacity=0.55, forget plot]
        coordinates {(0,2.35) (100,2.35)};

        \end{axis}

    \end{tikzpicture}
    }

    \caption{
    Inference trajectories of the #2 agent in twelve non-parametric tasks.
    Dashed lines indicate the corresponding ground-truth targets.
    }

    \label{fig:#3_multi_inference}
\end{figure}
}

\PlotDPMMAgentInference{dpmm_ant}{DPMM-Ant}{dpmm_ant}
\PlotDPMMAgentInference{dpmm_cheetah}{DPMM-Cheetah}{dpmm_cheetah}
\PlotDPMMAgentInference{dpmm_walker}{DPMM-Walker}{dpmm_walker}
\PlotDPMMAgentInference{dpmm_hopper}{DPMM-Hopper}{dpmm_hopper}
